Search for Spatially Extended Fermi-LAT Sources Using Two Years of Data

Spatial extension is an important characteristic for correctly associating gamma-ray-emitting sources with their counterparts at other wavelengths and for obtaining an unbiased model of their spectra. We present a new method for quantifying the spatial extension of sources detected by the Large Area Telescope (LAT), the primary science instrument on the Fermi Gamma-ray Space Telescope (Fermi). We perform a series of Monte Carlo simulations to validate this tool and calculate the LAT threshold for detecting the spatial extension of sources. We then test all sources in the second Fermi-LAT catalog (2FGL) for extension. We report the detection of seven new spatially extended sources.

==> Makefile <==
base = extended_search
extended_search:
#	pdflatex extended_search
#	bibtex extended_search
#	pdflatex extended_search
#	pdflatex extended_search
	latex $(base)
	bibtex $(base) 
	latex  $(base)
	latex  $(base)
	dvips $(base)
	# These commands make sure no compression is applied
	# # http://cosmocoffee.info/viewtopic.php?p=213
	ps2pdf -dAutoFilterColorImages=false -dColorImageFilter=/FlateEncode $(base).ps

clean:
	-rm -f $(base).aux $(base).log $(base).out \
      $(base).toc $(base).dvi $(base).bbl \
      $(base).blg $(base).ps


